Anomalous Entropic Behavior Observed in Quasar 3C 273

We investigate the flux intensities spanning from radio waves to $\gamma$-rays across 36 light curves of Quasar 3C 273, utilizing publicly available data collected by the Integral Science Data Centre (ISDC) database. Our analysis reveals a consistent adherence of all light curves from this quasar to $q$-Gaussian distribution. This compelling finding strongly suggests a nonextensive behavior exhibited by Quasar 3C 273. Moreover, we derive the $q$ entropic indices for these light curves, providing insights into the degree of nonextensivity, where cases with $q>1$ were primarily observed. Utilizing this index, we estimate the nonextensive entropy ($S_{q}$) and explore its correlation with the energy (in eV) and the $q$ index. Notably, we observe a tendency for the $q$ value to increase as the Tsallis entropy decreases. Remarkably, our most significant observation pertains to the relationship between the entropy $S_{q}$ and the energy of the source. We identify an anomalous behavior in entropy, particularly evident in the infrared and $\gamma$-ray wavebands.

==> resto.tex <==
Active Galactic Nuclei (AGNs) are known to be extremely bright and highly variable in multi-wavelengths \citep[e.g.][]{1995PASP..107..803U,1979ApJ...232...34B}. The bright and nearby radio-loud quasar 3C 273 (V = 12.85, z = 0.158)\citep{1963Natur..197}, whose flux curves have been largely studied at all frequencies for a few decades \citep[e.g.][]{2008MmSAI..79.1011C,1990A&A...234...73C,1987A&A...176..197C}, is one of the most featured examples of AGNs variability, presenting to date one of the most complete multi-wavelength databases available for an AGN. Thanks to the Integral Science Data Centre (ISDC) database\footnote{\url{http://www.isdc.unige.ch/3c273/}}, 3C 273 (alias 1226+023) has now available some 70 light curves, from radio to $\gamma$--ray wavebands, covering more than 40 years of observations \citep{2008A&A...486..411S,1999A&AS..134...89T}. Other datasets are found in the High-Energy Astrophysics Virtually ENlighted Sky (HEAVENS) web interface\footnote{\url{http://www.isdc.unige.ch/heavens/}} \citep{2010int..workE.162W} where several observations obtained by the instruments IBIS, SPI, JEM-X on board INTEGRAL, PCA on board RXTE \citep{1996SPIE.2808...59J}, and LAT on board {\it Fermi} \citep{2009ApJ...697.1071A} are also available to analyse the variability of quasar 3C 273 at high energies (from keV to GeV). 

Different procedures have been used to quantify the amplitude and periodicity of the AGNs variability, revealing a complex emission behaviour, which is believed to be due, at least partially, to the presence of multiple emission components produced by different root-causes, probably originating in different locations within the AGN \citep[e.g.][]{2008A&A...486..411S}. Quasi-periodic and periodic variations from the light curves of those objects have been widely studied. \citet{2015Natur.518...74G} report that a binary system of two supermassive black holes is suspected when the quasar shows periodic oscillations. However, low signal/noise of the data, irregular time sampling, instrumental effects are some factors, among others, to one consider a false periodicity as a real one \citep{2006AdSpR..38.1405V}. \citet{2016MNRAS.461.3145V} discuss stochastic models for periodic signals in order to control false periodicities detection. Many procedures, as the discrete autocorrelation function (DCF), the Lomb-Scargle periodogram and the wavelet transform (WT), have been employed to study the quasi-periodic and periodic variability of AGN sources \citep{2007A&A...469..899H,2006A&A...456L...1K,1998ApJ...503..662H}. Although, their behaviour could change over the years, suffering the effects of some transient phenomena within or around such astronomical objects.

Over the years, there are many reports of wavelet analysis of the quasar 3C 273, some of them considering few data points according to data availability, others focusing on a particular spectral emission and wavelength or on a specific kind of variability. Hence, this paper provides the largest time series data sample studied by wavelets up to date. We analyse 35 flux curves with a higher number of good data points from radio to $\gamma$--ray wavebands, in the search for unambiguous long- and short-scale periodicities.
